Critical dephasing rates for the observation of collective behavior in a pair of coupled quantum emitters

Efficient atom-photon interfaces require the controlled assembly of quantum emitters, where collective effects such as superradiance and subradiance can emerge. Recent experiments with subwavelength arrays of quantum dots have reported superradiance at room temperature, revealing a delicate competition between collective enhancement of coherent emission and pure dephasing $\gamma^*$, which destroys it. Motivated by these results, we theoretically study $N=2$ coupled quantum emitters and identify threshold values of $\gamma^*$, for four experimentally accessible observables, beyond which collective effects vanish. The thresholds depend sensitively on the chosen observable, highlighting the subtlety of detecting collective behavior. Our work provides a quantitative framework to guide experiments and optimize conditions for observing collective quantum phenomena.

==> figures/tikz/emitter_geometry.tex <==
\begin{tikzpicture}

% basis
\draw[->, thick] (0,0) -- (0,1) node[right] {$\hat{e}_z$};
\draw[->, thick] (0,0) -- (1,0) node[below] {$\hat{e}_x$};

\draw (0,0) circle (0.141) node[below right] {$\hat{e}_y$} node[below left] {$O$};
% e_y cross
\draw (-0.1,-0.1) -- (0.1,0.1);
\draw (0.1,-0.1) -- (-0.1,0.1);

%% emitter 1
\draw[->, very thick] (-2,0) -- (-2,1) node[below right] {$\hat{d}_1$};
% cross
\draw (-2-0.1,-0.1) -- (-2+0.1,0.1);
\draw (-2+0.1,-0.1) -- (-2-0.1,0.1);

%% emitter 2
\draw[->, very thick] (2,0) -- (2,1) node[below right] {$\hat{d}_2$};
% cross
\draw (2-0.1,-0.1) -- (2+0.1,0.1);
\draw (2+0.1,-0.1) -- (2-0.1,0.1);

%% r hat vector
\draw[->, thick] (-2,0) -- (-1,0) node[below] {$\hat{r}$};

\draw[|-|, thick] (-2,-0.8) -- node[below] {$r$} (2, -0.8);

%% r distance
\end{tikzpicture}
